Unveil Inversion and Invariance in Flow Transformer for Versatile Image Editing

Leveraging the large generative prior of the flow transformer for tuning-free image editing requires authentic inversion to project the image into the model's domain and a flexible invariance control mechanism to preserve non-target contents. However, the prevailing diffusion inversion performs deficiently in flow-based models, and the invariance control cannot reconcile diverse rigid and non-rigid editing tasks. To address these, we systematically analyze the \textbf{inversion and invariance} control based on the flow transformer. Specifically, we unveil that the Euler inversion shares a similar structure to DDIM yet is more susceptible to the approximation error. Thus, we propose a two-stage inversion to first refine the velocity estimation and then compensate for the leftover error, which pivots closely to the model prior and benefits editing. Meanwhile, we propose the invariance control that manipulates the text features within the adaptive layer normalization, connecting the changes in the text prompt to image semantics. This mechanism can simultaneously preserve the non-target contents while allowing rigid and non-rigid manipulation, enabling a wide range of editing types such as visual text, quantity, facial expression, etc. Experiments on versatile scenarios validate that our framework achieves flexible and accurate editing, unlocking the potential of the flow transformer for versatile image editing.

==> tabs/3_abla_inv.tex <==


\begin{table}[t]
\caption{{\bf Ablation Study on the fixed point iteration number and velocity compensation.} We choose a different iteration number to validate its effectiveness on editing.}
\begin{center}
  \resizebox{0.49\textwidth}{!}{
\begin{tabular}{@{}l|cccc@{}}
\toprule
Metric & Iter 1               & Iter 2               & Iter 3               & CP                   \\ \midrule
PSNR   &                      &                      &                      &                      \\ \midrule
MSE    &                      &                      &                      &                      \\ \midrule
LPIPS  &                      &                      &                      &                      \\ \midrule
SSIM   & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \midrule
CLIP   & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \midrule
CLIP   & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \bottomrule
\end{tabular}
}
\end{center}
\end{table}
